TurkBench: A Benchmark for Evaluating Turkish Large Language Models

With the recent surge in the development of large language models, the need for comprehensive and language-specific evaluation benchmarks has become critical. While significant progress has been made in evaluating English-language models, benchmarks for other languages, particularly those with unique linguistic characteristics such as Turkish, remain less developed. Our study introduces TurkBench, a comprehensive benchmark designed to assess the capabilities of generative large language models in the Turkish language. TurkBench involves 8,151 data samples across 21 distinct subtasks. These are organized under six main categories of evaluation: Knowledge, Language Understanding, Reasoning, Content Moderation, Turkish Grammar and Vocabulary, and Instruction Following. The diverse range of tasks and the culturally relevant data would provide researchers and developers with a valuable tool for evaluating their models and identifying areas for improvement. We further publish our benchmark for online submissions at https://huggingface.co/turkbench

==> main <==
@misc{ponti2020xcopamultilingualdatasetcausal,
      title={XCOPA: A Multilingual Dataset for Causal Commonsense Reasoning}, 
      author={Edoardo Maria Ponti and Goran Glavaš and Olga Majewska and Qianchu Liu and Ivan Vulić and Anna Korhonen},
      year={2020},
      eprint={2005.00333},
      archivePrefix={arXiv},
      primaryClass={cs.CL},
      url={https://arxiv.org/abs/2005.00333}, 
}


@misc{alpaca_2023,
  author       = {Taori, Rohan and Gulrajani, Ishaan and Zhang, Tianyi and Dubois, Yann and Li, Xuechen and Guestrin, Carlos and Liang, Percy and Hashimoto, Tatsunori B.},
  title        = {Alpaca: A Strong, Replicable Instruction‑Following Model},
  howpublished = {Blog post, Stanford Center for Research on Foundation Models},
  month        = mar,
  year         = {2023},
  url          = {https://crfm.stanford.edu/2023/03/13/alpaca.html},
  note         = {Accessed: 2025‑06‑25},
}

@article{parrish2021bbq,
  title={BBQ: A hand-built bias benchmark for question answering},
  author={Parrish, Alicia and Chen, Angelica and Nangia, Nikita and Padmakumar, Vishakh and Phang, Jason and Thompson, Jana and Htut, Phu Mon and Bowman, Samuel R},
  journal={arXiv preprint arXiv:2110.08193},
  year={2021}
}

@article{lin2021truthfulqa,
  title={Truthfulqa: Measuring how models mimic human falsehoods},
  author={Lin, Stephanie and Hilton, Jacob and Evans, Owain},
  journal={arXiv preprint arXiv:2109.07958},
  year={2021}
}

@article{DBLP:journals/corr/abs-2009-03300,
  author       = {Dan Hendrycks and
                  Collin Burns and
                  Steven Basart and
                  Andy Zou and
                  Mantas Mazeika and
                  Dawn Song and
                  Jacob Steinhardt},
  title        = {Measuring Massive Multitask Language Understanding},
  journal      = {CoRR},
  volume       = {abs/2009.03300},
  year         = {2020},
  url          = {https://arxiv.org/abs/2009.03300},
  eprinttype    = {arXiv},
  eprint       = {2009.03300},
  timestamp    = {Thu, 17 Sep 2020 12:49:52 +0200},
  biburl       = {https://dblp.org/rec/journals/corr/abs-2009-03300.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{umutlu-etal-2025-evaluating,
    title = "Evaluating the Quality of Benchmark Datasets for Low-Resource Languages: A Case Study on {T}urkish",
    author = "Umutlu, Elif Ecem  and
      Cengiz, Ayse Aysu  and
      Sever, Ahmet Kaan  and
      Erdem, Seyma  and
      Aytan, Burak  and
      Tufan, Busra  and
      Topraksoy, Abdullah  and
      Dar{\i}c{\i}, Esra  and
      Toraman, Cagri",
    editor = "Arviv, Ofir  and
      Clinciu, Miruna  and
      Dhole, Kaustubh  and
      Dror, Rotem  and
      Gehrmann, Sebastian  and
      Habba, Eliya  and
      Itzhak, Itay  and
      Mille, Simon  and
      Perlitz, Yotam  and
      Santus, Enrico  and
      Sedoc, Jo{\~a}o  and
      Shmueli Scheuer, Michal  and
      Stanovsky, Gabriel  and
      Tafjord, Oyvind",
    booktitle = "Proceedings of the Fourth Workshop on Generation, Evaluation and Metrics (GEM{\texttwosuperior})",
    month = jul,
    year = "2025",
    address = "Vienna, Austria and virtual meeting",
    publisher = "Association for Computational Linguistics",
    url = "https://aclanthology.org/2025.gem-1.41/",
    pages = "471--487",
    ISBN = "979-8-89176-261-9",
    abstract = "The reliance on translated or adapted datasets from English or multilingual resources introduces challenges regarding linguistic and cultural suitability. This study addresses the need for robust and culturally appropriate benchmarks by evaluating the quality of 17 commonly used Turkish benchmark datasets. Using a comprehensive framework that assesses six criteria, both human and LLM-judge annotators provide detailed evaluations to identify dataset strengths and shortcomings.Our results reveal that 70{\%} of the benchmark datasets fail to meet our heuristic quality standards. The correctness of the usage of technical terms is the strongest criterion, but 85{\%} of the criteria are not satisfied in the examined datasets. Although LLM judges demonstrate potential, they are less effective than human annotators, particularly in understanding cultural common sense knowledge and interpreting fluent, unambiguous text. GPT-4o has stronger labeling capabilities for grammatical and technical tasks, while Llama3.3-70B excels at correctness and cultural knowledge evaluation. Our findings emphasize the urgent need for more rigorous quality control in creating and adapting datasets for low-resource languages."
}

@inproceedings{wang-etal-2018-glue,
    title = "{GLUE}: A Multi-Task Benchmark and Analysis Platform for Natural Language Understanding",
    author = "Wang, Alex  and
      Singh, Amanpreet  and
      Michael, Julian  and
      Hill, Felix  and
      Levy, Omer  and
      Bowman, Samuel",
    editor = "Linzen, Tal  and
      Chrupa{\l}a, Grzegorz  and
      Alishahi, Afra",
    booktitle = "Proceedings of the 2018 {EMNLP} Workshop {B}lackbox{NLP}: Analyzing and Interpreting Neural Networks for {NLP}",
    month = nov,
    year = "2018",
    address = "Brussels, Belgium",
    publisher = "Association for Computational Linguistics",
    url = "https://aclanthology.org/W18-5446/",
    doi = "10.18653/v1/W18-5446",
    pages = "353--355",
    abstract = "Human ability to understand language is \textit{general, flexible, and robust}. In contrast, most NLU models above the word level are designed for a specific task and struggle with out-of-domain data. If we aspire to develop models with understanding beyond the detection of superficial correspondences between inputs and outputs, then it is critical to develop a unified model that can execute a range of linguistic tasks across different domains. To facilitate research in this direction, we present the General Language Understanding Evaluation (GLUE, gluebenchmark.com): a benchmark of nine diverse NLU tasks, an auxiliary dataset for probing models for understanding of specific linguistic phenomena, and an online platform for evaluating and comparing models. For some benchmark tasks, training data is plentiful, but for others it is limited or does not match the genre of the test set. GLUE thus favors models that can represent linguistic knowledge in a way that facilitates sample-efficient learning and effective knowledge-transfer across tasks. While none of the datasets in GLUE were created from scratch for the benchmark, four of them feature privately-held test data, which is used to ensure that the benchmark is used fairly. We evaluate baselines that use ELMo (Peters et al., 2018), a powerful transfer learning technique, as well as state-of-the-art sentence representation models. The best models still achieve fairly low absolute scores. Analysis with our diagnostic dataset yields similarly weak performance over all phenomena tested, with some exceptions."
}

@inproceedings{NEURIPS2019_4496bf24,
 author = {Wang, Alex and Pruksachatkun, Yada and Nangia, Nikita and Singh, Amanpreet and Michael, Julian and Hill, Felix and Levy, Omer and Bowman, Samuel},
 booktitle = {Advances in Neural Information Processing Systems},
 editor = {H. Wallach and H. Larochelle and A. Beygelzimer and F. d\textquotesingle Alch\'{e}-Buc and E. Fox and R. Garnett},
 pages = {},
 publisher = {Curran Associates, Inc.},
 title = {SuperGLUE: A Stickier Benchmark for General-Purpose Language Understanding Systems},
 url = {https://proceedings.neurips.cc/paper_files/paper/2019/file/4496bf24afe7fab6f046bf4923da8de6-Paper.pdf},
 volume = {32},
 year = {2019}
}

@article{hendryckstest2021,
  title={Measuring Massive Multitask Language Understanding},
  author={Dan Hendrycks and Collin Burns and Steven Basart and Andy Zou and Mantas Mazeika and Dawn Song and Jacob Steinhardt},
  journal={Proceedings of the International Conference on Learning Representations (ICLR)},
  year={2021}
}


@inproceedings{lai-etal-2024-llms,
    title = "{LLM}s Beyond {E}nglish: Scaling the Multilingual Capability of {LLM}s with Cross-Lingual Feedback",
    author = "Lai, Wen  and
      Mesgar, Mohsen  and
      Fraser, Alexander",
    editor = "Ku, Lun-Wei  and
      Martins, Andre  and
      Srikumar, Vivek",
    booktitle = "Findings of the Association for Computational Linguistics: ACL 2024",
    month = aug,
    year = "2024",
    address = "Bangkok, Thailand",
    publisher = "Association for Computational Linguistics",
    url = "https://aclanthology.org/2024.findings-acl.488/",
    doi = "10.18653/v1/2024.findings-acl.488",
    pages = "8186--8213",
    abstract = "To democratize large language models (LLMs) to most natural languages, it is imperative to make these models capable of understanding and generating texts in many languages, in particular low-resource ones. While recent multilingual LLMs demonstrate remarkable performance in such capabilities, these LLMs still support a limited number of human languages due to the lack of training data for low resource languages. Moreover, these LLMs are not yet aligned with human preference for downstream tasks, which is crucial for the success of LLMs in English. In this paper, we introduce xLLaMA-100 and xBLOOM-100 (collectively xLLMs-100), which scale the multilingual capabilities of LLaMA and BLOOM to 100 languages. To do so, we construct two datasets: a multilingual instruction dataset including 100 languages, which represents the largest language coverage to date, and a cross-lingual human feedback dataset encompassing 30 languages. We perform multilingual instruction tuning on the constructed instruction data and further align the LLMs with human feedback using the DPO algorithm on our cross-lingual human feedback dataset. We evaluate the multilingual understanding and generating capabilities of xLLMs-100 on five multilingual benchmarks. Experimental results show that xLLMs-100 consistently outperforms its peers across the benchmarks by considerable margins, defining a new state-of-the-art multilingual LLM that supports 100 languages."
}

@article{hakkani2002statistical,
  title={Statistical morphological disambiguation for agglutinative languages},
  author={Hakkani-T{\"u}r, Dilek Z and Oflazer, Kemal and T{\"u}r, G{\"o}khan},
  journal={Computers and the Humanities},
  volume={36},
  number={4},
  pages={381--410},
  year={2002},
  publisher={Springer}
}

@article{oflazer2014turkish,
  title={Turkish and its challenges for language processing},
  author={Oflazer, Kemal},
  journal={Language resources and evaluation},
  volume={48},
  number={4},
  pages={639--653},
  year={2014},
  publisher={Springer}
}

@inproceedings{nacar2025towards,
  title={Towards inclusive Arabic LLMs: A culturally aligned benchmark in Arabic large language model evaluation},
  author={Nacar, Omer and Sibaee, Serry Taiseer and Ahmed, Samar and Atitallah, Safa Ben and Ammar, Adel and Alhabashi, Yasser and Al-Batati, Abdulrahman S and Alsehibani, Arwa and Qandos, Nour and Elshehy, Omar and others},
  booktitle={Proceedings of the First Workshop on Language Models for Low-Resource Languages},
  pages={387--401},
  year={2025}
}

@inproceedings{baucells2025iberobench,
  title={Iberobench: A benchmark for llm evaluation in iberian languages},
  author={Baucells, Irene and Aula-Blasco, Javier and de-Dios-Flores, Iria and Su{\'a}rez, Silvia Paniagua and Perez, Naiara and Salles, Anna and Docio, Susana Sotelo and Falc{\~a}o, J{\'u}lia and Saiz, Jos{\'e} Javier and Sep{\'u}lveda-Torres, Robiert and others},
  booktitle={Proceedings of the 31st International Conference on Computational Linguistics},
  pages={10491--10519},
  year={2025}
}

@inproceedings{magnini2025leaderboard,
  title={A Leaderboard for Benchmarking LLMs on Italian},
  author={Magnini, Bernardo and Madeddu, Marco and Resta, Michele and Zanoli, Roberto and Cimmino, Martin and Albano, Paolo and Patti, Viviana},
  booktitle={Proceedings of the Eleventh Italian Conference on Computational Linguistics (CLiC-it 2025)},
  pages={636--646},
  year={2025}
}

@inproceedings{park-etal-2024-open,
    title = "Open {K}o-{LLM} Leaderboard: Evaluating Large Language Models in {K}orean with {K}o-H5 Benchmark",
    author = "Park, Chanjun  and
      Kim, Hyeonwoo  and
      Kim, Dahyun  and
      Cho, SeongHwan  and
      Kim, Sanghoon  and
      Lee, Sukyung  and
      Kim, Yungi  and
      Lee, Hwalsuk",
    editor = "Ku, Lun-Wei  and
      Martins, Andre  and
      Srikumar, Vivek",
    booktitle = "Proceedings of the 62nd Annual Meeting of the Association for Computational Linguistics (Volume 1: Long Papers)",
    month = aug,
    year = "2024",
    address = "Bangkok, Thailand",
    publisher = "Association for Computational Linguistics",
    url = "https://aclanthology.org/2024.acl-long.177/",
    doi = "10.18653/v1/2024.acl-long.177",
    pages = "3220--3234",
    abstract = "This paper introduces the Open Ko-LLM Leaderboard and the Ko-H5 Benchmark as vital tools for evaluating Large Language Models (LLMs) in Korean. Incorporating private test sets while mirroring the English Open LLM Leaderboard, we establish a robust evaluation framework that has been well integrated in the Korean LLM community. We perform data leakage analysis that shows the benefit of private test sets along with a correlation study within the Ko-H5 benchmark and temporal analyses of the Ko-H5 score. Moreover, we present empirical support for the need to expand beyond set benchmarks. We hope the Open Ko-LLM Leaderboard sets precedent for expanding LLM evaluation to foster more linguistic diversity."
}

@article{zheng2023judging,
  title={Judging llm-as-a-judge with mt-bench and chatbot arena},
  author={Zheng, Lianmin and Chiang, Wei-Lin and Sheng, Ying and Zhuang, Siyuan and Wu, Zhanghao and Zhuang, Yonghao and Lin, Zi and Li, Zhuohan and Li, Dacheng and Xing, Eric and others},
  journal={Advances in neural information processing systems},
  volume={36},
  pages={46595--46623},
  year={2023}
}

@article{liang2022holistic,
  title={Holistic evaluation of language models},
  author={Liang, Percy and Bommasani, Rishi and Lee, Tony and Tsipras, Dimitris and Soylu, Dilara and Yasunaga, Michihiro and Zhang, Yian and Narayanan, Deepak and Wu, Yuhuai and Kumar, Ananya and others},
  journal={arXiv preprint arXiv:2211.09110},
  year={2022}
}

@article{zheng2023judging,
  title={Judging llm-as-a-judge with mt-bench and chatbot arena},
  author={Zheng, Lianmin and Chiang, Wei-Lin and Sheng, Ying and Zhuang, Siyuan and Wu, Zhanghao and Zhuang, Yonghao and Lin, Zi and Li, Zhuohan and Li, Dacheng and Xing, Eric and others},
  journal={Advances in neural information processing systems},
  volume={36},
  pages={46595--46623},
  year={2023}
}

@article{srivastava2022beyond,
  title={Beyond the Imitation Game: Quantifying and extrapolating the capabilities of language models},
  author={Srivastava, Aarohi and Rastogi, Abhinav and Rao, Abhishek and Shoeb, Abu Awal Md and Abid, Abubakar and Fisch, Adam and Brown, Adam R and Santoro, Adam and Gupta, Aditya and Garriga-Alonso, Adri{\`a} and others},
  journal={arXiv preprint arXiv:2206.04615},
  year={2022}
}

@inproceedings{lin-etal-2022-truthfulqa,
    title = "{T}ruthful{QA}: Measuring How Models Mimic Human Falsehoods",
    author = "Lin, Stephanie  and
      Hilton, Jacob  and
      Evans, Owain",
    editor = "Muresan, Smaranda  and
      Nakov, Preslav  and
      Villavicencio, Aline",
    booktitle = "Proceedings of the 60th Annual Meeting of the Association for Computational Linguistics (Volume 1: Long Papers)",
    month = may,
    year = "2022",
    address = "Dublin, Ireland",
    publisher = "Association for Computational Linguistics",
    url = "https://aclanthology.org/2022.acl-long.229/",
    doi = "10.18653/v1/2022.acl-long.229",
    pages = "3214--3252",
    abstract = "We propose a benchmark to measure whether a language model is truthful in generating answers to questions. The benchmark comprises 817 questions that span 38 categories, including health, law, finance and politics. We crafted questions that some humans would answer falsely due to a false belief or misconception. To perform well, models must avoid generating false answers learned from imitating human texts. We tested GPT-3, GPT-Neo/J, GPT-2 and a T5-based model. The best model was truthful on 58{\%} of questions, while human performance was 94{\%}. Models generated many false answers that mimic popular misconceptions and have the potential to deceive humans. The largest models were generally the least truthful. This contrasts with other NLP tasks, where performance improves with model size. However, this result is expected if false answers are learned from the training distribution. We suggest that scaling up models alone is less promising for improving truthfulness than fine-tuning using training objectives other than imitation of text from the web."
}

@inproceedings{hu2020xtreme,
  title={Xtreme: A massively multilingual multi-task benchmark for evaluating cross-lingual generalisation},
  author={Hu, Junjie and Ruder, Sebastian and Siddhant, Aditya and Neubig, Graham and Firat, Orhan and Johnson, Melvin},
  booktitle={International conference on machine learning},
  pages={4411--4421},
  year={2020},
  organization={PMLR}
}

@inproceedings{liang-etal-2020-xglue,
    title = "{XGLUE}: A New Benchmark Dataset for Cross-lingual Pre-training, Understanding and Generation",
    author = "Liang, Yaobo  and
      Duan, Nan  and
      Gong, Yeyun  and
      Wu, Ning  and
      Guo, Fenfei  and
      Qi, Weizhen  and
      Gong, Ming  and
      Shou, Linjun  and
      Jiang, Daxin  and
      Cao, Guihong  and
      Fan, Xiaodong  and
      Zhang, Ruofei  and
      Agrawal, Rahul  and
      Cui, Edward  and
      Wei, Sining  and
      Bharti, Taroon  and
      Qiao, Ying  and
      Chen, Jiun-Hung  and
      Wu, Winnie  and
      Liu, Shuguang  and
      Yang, Fan  and
      Campos, Daniel  and
      Majumder, Rangan  and
      Zhou, Ming",
    editor = "Webber, Bonnie  and
      Cohn, Trevor  and
      He, Yulan  and
      Liu, Yang",
    booktitle = "Proceedings of the 2020 Conference on Empirical Methods in Natural Language Processing (EMNLP)",
    month = nov,
    year = "2020",
    address = "Online",
    publisher = "Association for Computational Linguistics",
    url = "https://aclanthology.org/2020.emnlp-main.484/",
    doi = "10.18653/v1/2020.emnlp-main.484",
    pages = "6008--6018",
    abstract = "In this paper, we introduce XGLUE, a new benchmark dataset to train large-scale cross-lingual pre-trained models using multilingual and bilingual corpora, and evaluate their performance across a diverse set of cross-lingual tasks. Comparing to GLUE (Wang et al.,2019), which is labeled in English and includes natural language understanding tasks only, XGLUE has three main advantages: (1) it provides two corpora with different sizes for cross-lingual pre-training; (2) it provides 11 diversified tasks that cover both natural language understanding and generation scenarios; (3) for each task, it provides labeled data in multiple languages. We extend a recent cross-lingual pre-trained model Unicoder (Huang et al., 2019) to cover both understanding and generation tasks, which is evaluated on XGLUE as a strong baseline. We also evaluate the base versions (12-layer) of Multilingual BERT, XLM and XLM-R for comparison."
}

@article{baysan2025tr,
  title={TR-MTEB: A Comprehensive Benchmark and Embedding Model Suite for Turkish Sentence Representations},
  author={Baysan, Mehmet Selman and Bebek, Istanbul and G{\"u}ng{\"o}r, Tunga},
  journal={C. Christodoulopoulos, T. Chakraborty, C. Rose, \& V. Peng (Eds), Findings of the Association for Computational Linguistics: EMNLP 2025},
  pages={8867--8887},
  year={2025}
}

@inproceedings{uzunouglu2023benchmarking,
  title={Benchmarking procedural language understanding for low-resource languages: A case study on Turkish},
  author={Uzuno{\u{g}}lu, Arda and {\c{S}}ahin, G{\"o}zde G{\"u}l},
  booktitle={Proceedings of the 13th International Joint Conference on Natural Language Processing and the 3rd Conference of the Asia-Pacific Chapter of the Association for Computational Linguistics (Volume 1: Long Papers)},
  pages={804--819},
  year={2023}
}

@article{warstadt2020blimp,
  title={BLiMP: The benchmark of linguistic minimal pairs for English},
  author={Warstadt, Alex and Parrish, Alicia and Liu, Haokun and Mohananey, Anhad and Peng, Wei and Wang, Sheng-Fu and Bowman, Samuel R},
  journal={Transactions of the Association for Computational Linguistics},
  volume={8},
  pages={377--392},
  year={2020},
  publisher={MIT Press One Rogers Street, Cambridge, MA 02142-1209, USA journals-info~…}
}

@inproceedings{gauthier2020syntaxgym,
  title={SyntaxGym: An online platform for targeted evaluation of language models},
  author={Gauthier, Jon and Hu, Jennifer and Wilcox, Ethan and Qian, Peng and Levy, Roger},
  booktitle={Proceedings of the 58th Annual Meeting of the Association for Computational Linguistics: System Demonstrations},
  pages={70--76},
  year={2020}
}

@inproceedings{ates2022craft,
  title={Craft: A benchmark for causal reasoning about forces and interactions},
  author={Ates, Tayfun and Ate{\c{s}}o{\u{g}}lu, M and Yi{\u{g}}it, {\c{C}}a{\u{g}}atay and Kesen, Ilker and Kobas, Mert and Erdem, Erkut and Erdem, Aykut and Goksun, Tilbe and Yuret, Deniz},
  booktitle={Findings of the Association for Computational Linguistics: ACL 2022},
  pages={2602--2627},
  year={2022}
}

@article{ccoltekin2023resources,
  title={Resources for Turkish natural language processing: A critical survey},
  author={{\c{C}}{\"o}ltekin, {\c{C}}a{\u{g}}r{\i} and Do{\u{g}}ru{\"o}z, A Seza and {\c{C}}etino{\u{g}}lu, {\"O}zlem},
  journal={Language Resources and Evaluation},
  volume={57},
  number={1},
  pages={449--488},
  year={2023},
  publisher={Springer}
}

@article{er2025cetvel,
  title={Cetvel: A Unified Benchmark for Evaluating Language Understanding, Generation and Cultural Capacity of LLMs for Turkish},
  author={Er, Yakup Abrek and Kesen, Ilker and {\c{S}}ahin, G{\"o}zde G{\"u}l and Erdem, Aykut},
  journal={arXiv preprint arXiv:2508.16431},
  year={2025}
}

@inproceedings{yuksel2024turkishmmlu,
  title={Turkishmmlu: Measuring massive multitask language understanding in turkish},
  author={Y{\"u}ksel, Arda and K{\"o}ksal, Abdullatif and Senel, L{\"u}tfi Kerem and Korhonen, Anna and Sch{\"u}tze, Hinrich},
  booktitle={Findings of the Association for Computational Linguistics: EMNLP 2024},
  pages={7035--7055},
  year={2024}
}

@inproceedings{bayram2025tr,
  title={TR-MMLU Benchmark for Large Language Models: Performance Evaluation, Challenges, and Opportunities for Improvement},
  author={Bayram, M Ali and Fincan, Ali Arda and G{\"u}m{\"u}{\c{s}}, Ahmet Semih and Diri, Banu and Y{\i}ld{\i}r{\i}m, Sava{\c{s}} and Ayta{\c{s}}, {\"O}ner},
  booktitle={2025 33rd Signal Processing and Communications Applications Conference (SIU)},
  pages={1--4},
  year={2025},
  organization={IEEE}
}

@inproceedings{acikgoz-etal-2024-bridging,
    title = "Bridging the Bosphorus: Advancing {T}urkish Large Language Models through Strategies for Low-Resource Language Adaptation and Benchmarking",
    author = "Acikgoz, Emre Can  and
      Erdogan, Mete  and
      Yuret, Deniz",
    editor = {S{\"a}lev{\"a}, Jonne  and
      Owodunni, Abraham},
    booktitle = "Proceedings of the Fourth Workshop on Multilingual Representation Learning (MRL 2024)",
    month = nov,
    year = "2024",
    address = "Miami, Florida, USA",
    publisher = "Association for Computational Linguistics",
    url = "https://aclanthology.org/2024.mrl-1.21/",
    doi = "10.18653/v1/2024.mrl-1.21",
    pages = "242--268",
}

@inproceedings{toraman-2024-adapting,
    title = "Adapting Open-Source Generative Large Language Models for Low-Resource Languages: A Case Study for {T}urkish",
    author = "Toraman, Cagri",
    editor = {S{\"a}lev{\"a}, Jonne  and
      Owodunni, Abraham},
    booktitle = "Proceedings of the Fourth Workshop on Multilingual Representation Learning (MRL 2024)",
    month = nov,
    year = "2024",
    address = "Miami, Florida, USA",
    publisher = "Association for Computational Linguistics",
    url = "https://aclanthology.org/2024.mrl-1.3/",
    doi = "10.18653/v1/2024.mrl-1.3",
    pages = "30--44",
}
